Geometric Exploration for Online Control

We study the control of an \emph{unknown} linear dynamical system under general convex costs. The objective is minimizing regret vs. the class of disturbance-feedback-controllers, which encompasses all stabilizing linear-dynamical-controllers. In this work, we first consider the case of known cost functions, for which we design the first polynomial-time algorithm with $n^3\sqrt{T}$-regret, where $n$ is the dimension of the state plus the dimension of control input. The $\sqrt{T}$-horizon dependence is optimal, and improves upon the previous best known bound of $T^{2/3}$. The main component of our algorithm is a novel geometric exploration strategy: we adaptively construct a sequence of barycentric spanners in the policy space. Second, we consider the case of bandit feedback, for which we give the first polynomial-time algorithm with $poly(n)\sqrt{T}$-regret, building on Stochastic Bandit Convex Optimization.

==> New_ideas.tex <==

\subsection{Our  Approach and New Techniques }


The cost $J(K)$ is nonconvex in $K$. To remedy this, we use an alternative disturbance-based policy class, introduced in \cite{agarwal2019online}, where the control is linear in the past disturbances (as opposed to the state): 
\begin{align}\label{eq:noise-based-policy}
  u_t=\sum_{i=1}^H M^{[i-1]}w_{t-i}, 
\end{align}
where $H$ is a hyperparameter.
This parameterization is useful, because the offline search for an optimal disturbance-based policy can be posed as a convex program.
In \cite{agarwal2019online}, the authors show that disturbance-based policies can approximate all strongly stable linear policies.  
We move on to describe the novel components of our work. 
\paragraph{Geometric exploration:} Algorithm \ref{LJ-exploration} runs in epochs and follows the phased-elimination paradigm \cite{lattimore_szepesvari_2020}. During epoch $r$, it focuses on a convex disturbance-based policy set $\mathcal{M}_r$, which by the end of the epoch will be substituted by $\mathcal{M}_{r+1}\subseteq \mathcal{M}_r$. 
In the beginning of the epoch, it decides on a set of \emph{exploratory policies} to be executed during the epoch. This is done by constructing a barycentric spanner of the policy set $\mathcal{M}_r$ (Definition \ref{def:barycentric}).
At the end of the epoch, it refines its estimates for the system matrices $A_*,B_*$ and creates $\mathcal{M}_{r+1}\subseteq \mathcal{M}_r$.
\paragraph{Estimating the disturbances:}
A typical difficulty in using disturbance-based policies is that we do not know the disturbances, and since the system matrices are unknown, we cannot recover $w_t$ by using $w_t=x_{t+1}-A_*x_t-B_*u_t$. A key contribution of this work is showing that \emph{disturbances can be accurately estimated, without accurately estimating the system matrices $A_*,B_*$}.
\paragraph{Coupling:} At the end of epoch $r$, we create estimates $\whA,\whB$ of $A_*,B_*$, which we use to create the next policy set $\mathcal{M}_{r+1}$. These estimates are not necessarily accurate in every direction. To argue that $\mathcal{M}_{r+1}$ contains good policies, we employ a probabilistic coupling argument between the true system and the estimated one. This could be a useful technique for future works.
\paragraph{Robustness of stochastic BCO:} For bandit feedback, we require a generalization of the Stochastc Bandit Convex Optimization (SBCO) framework, where the noise contains a small adversarial component in addition to the stochastic part. The need for robustness to adversarial noise arises from the estimation error on the disturbances $\|\widehat{w}_t-w_t\|$. %However, because of the noise-approximation analysis, these perturbations are small and the aforementioned algorithm can be used for control with bandit feedback.
We prove that by appropriately changing the parameters in the SBCO algorithm from \cite{agarwal2011stochastic}, we can get $\sqrt{T}$-regret for this more general model. 


==> Relaxation+Barycentric.tex <==
%\subsection{Background}\label{sec:cvx_relax}
\subsubsection{Disturbance-based policies}\label{subs:disturbance-policies}

The cost $J(K)$ is nonconvex in $K$. To remedy this, we use an alternative disturbance-based policy class, introduced in \cite{agarwal2019online}, where the control is linear in the past disturbances (as opposed to the state): 
\begin{align}\label{eq:noise-based-policy}
  u_t=\sum_{i=1}^H M^{[i-1]}w_{t-i}, 
\end{align}
where $H$ is a hyperparameter.
This parameterization is useful, because the offline search for an optimal disturbance-based policy can be posed as a convex program.
In \cite{agarwal2019online}, the authors show that disturbance-based policies can approximate all strongly stable linear policies.  
%Our algorithms will use noise-based policies, which were first introduced in \cite{agarwal2019online}. In this section we give the necessary background on noise-based policies, following \cite{hazan2019nonstochastic}. As we will see, the reasons to use this policy class is 1. it can approximately express all policies in $\mathcal{K}$, and 2. at any time $t$, the cost as a function of the policy is convex. 
Let $H:= C\cdot \gamma^{-1}\cdot \log{\left(Td_xd_u\kappa\beta\gamma^{-1}\right)}$, where $C$ is a sufficiently large constant (e.g., 1000). We provide some background definitions, introduced in \cite{agarwal2019online}.
\begin{definition}\label{def:controller}
A disturbance-based policy $M=\left(M^{[0]},\dots,M^{[H-1]}\right)$ applied at time $t$ chooses control $u_t=\sum_{i=1}^HM^{[i-1]}w_{t-i}$, where $w_s=0$, for $s\leq 0$.
\end{definition}
Under the execution of a disturbance-based policy $M$, the state can be expressed as $x_{t+1}=A_*^{H+1}x_{t-H}+\sum_{i=0}^{2H}\Psi_i(M\ |\ A_*,B_*)w_{t-i}$ \footnote{We set $x_s=0$, for $s\leq 0$.}, where $\Psi_i(M\ |\ A_*,B_*)$ is an affine function of $M$. We provide exact expressions for $\Psi_i$ in Appendix \ref{appdx:disturbance-based}. Because $A_*$ is $(\kappa,\gamma)$-strongly stable, it can be shown that $A_*^{H+1}\approx 0$. This leads to the definition of surrogate state $\ox_{t+1}=\sum_{i=0}^{2H}\Psi_i(M\ |\ A_*,B_*)w_{t-i}\approx x_{t+1}$. We now define a function that approximates very well the average infinite cost of executing $M$, without involving infinite limits that create computational issues. Let $t\geq 2H+2$. We define the stationary cost $\mathcal{C}\big(M\   |\ A_*, B_* \big)=\mathbb{E}_{w} \left[ c(\ox_t,u_t ) \right]$, where $w$ denotes the sequence $(w_t)_t$. Observe that the stationary cost does not depend on $t$, since $(\ox_t,u_t)$ have the same distribution for all $t\geq 2H+2$. Also, observe that $\mathcal{C}$ is a convex function of $M$, because $\ox_t$ and $u_t$ are affine in $M$ and $c$ is convex. We define the policy set $\mM=\left\{\left(M^{[0]},\dots,M^{[H-1]}\right) \ \Big|\ \left\|M^{[i]}\right\|\leq \kappa^3\beta (1-\gamma)^i \right\}$.
In \cite{agarwal2019online}, the authors proved that $\mM$ can approximately express all policies in $\mathcal{K}$, which is formally captured by Theorem \ref{thm:cvx_relax} in Appendix \ref{appdx:subs:express}. The algorithms we present in the paper aim to minimize the function $\mathcal{C}\left(M\   |\ A_*, B_* \right)$ over $\mM$. The difficulty is that we do not know this function, since we don't know $A_*,B_*$.
Under the execution of a disturbance-based policy $M$, the state can be expressed as an affine transformation $\Psi$ (defined below) of the disturbances, where transformation $\Psi$ is affine in the matrices of $M$.
By unrolling $x_{t+1}$, we get $x_{t+1}=A_*^{H+1}x_{t-H}+\sum_{i=0}^{2H}\Psi_i(M\ |\ A_*,B_*)w_{t-i}$ \footnote{We set $x_s=0$, for $s\leq 0$.}, where $\Psi_i(M\ |\ A_*,B_*)=A_*^{i}\ind_{i\leq H}+\sum_{j=0}^HA_*^j  
    B_* M^{[i-j-1]}\ind_{i-j\in[1,H]}.$\footnote{The expression $\ind_{i\leq k}$ is 1 if $i\leq k$ and 0 otherwise.} For completeness, we derive this formula in Appendix \ref{appdx:disturbance-based}.
%\begin{align}\label{eq:unroll}
 %   x_{t+1}=A_*^{H+1}x_{t-H}+\sum_{i=0}^{2H}\Psi_i(M\ |\ A_*,B_*)w_{t-i},
%\end{align}
%\begin{align}\label{eq:transfer}
 %  \Psi_i(M\ |\ A_*,B_*)=A_*^{i}\ind_{i\leq H}+\sum_{j=0}^HA_*^j  
  %  B_* M^{[i-j-1]}\ind_{i-j\in[1,H]}. \text{\footnotemark}
%\end{align}
\op{Do as icml}
\paragraph{Surrogate state and control:}\label{par:sur-state-control}
%When  It can be shown that $\|A_*^{H+1}\|$ is negligible and so it makes sense to
We define two time-independent quantities: surrogate state and surrogate control. Let $\eta=(\eta_0,\eta_1,\dots \eta_{2H})$, where  $\eta_i\simiid N(0,I)$. We define
$u\big(M\ |\ \eta\big)=\sum_{i=0}^{H-1}M^{[i]}\eta_i$ and $ x\big(M\ |\ A_*,B_*,\eta \big)=\sum_{i=0}^{2H}\Psi_i(M\ |\ A_*,B_*)\eta_i$. Because $A_*$ is $(\kappa,\gamma)$-strongly stable, it can be shown that $A_*^{H+1}\approx 0$, so when we execute policy $M$ and $t\geq \Omega(H)$, the state/control pair $(x_t,u_t)$ is almost identically distributed with $\left(x\big(M\ |\ A_*,B_*,\eta \big), u\big(M\ |\ \eta\big)\right)$. 
%The term in \ref{eq:unroll} that includes $A_*^{H+1}$ will be very small, due to Assumption \ref{assump:stability} and the choice of $H$. For large $t$, if this term is dropped, then the distribution of the RHS \ref{eq:unroll} is independent of $t$. We define the surrogate state and surrogate control. a policy $M$ and a sequence $w_{1:H}=(w_0,\dots,w_{2H})$ we define a surrogate state and surrogate control as follows.
%\includegraphics[width=\linewidth]{9.png}
%\begin{align}\label{eq:sur_state}
 %   x\big(M\ |\ A_*,B_*,\eta \big)=\sum_{i=0}^{2H}\Psi_i(M\ |\ A_*,B_*)\eta_i\ \ \ \ \text{and}\ \ \ u\big(M\ |\ \eta\big)=\sum_{i=0}^{H-1}M^{[i]}\eta_i.
%\end{align}
\paragraph{Convex stationary cost:} 
We define a function that approximates very well the average cost of executing $M$, i.e., $\mathcal{C}\big(M\   |\ A_*, B_* \big)=\mathbb{E}_{\eta} \Bigg[ c\Big(x(M\ |\ A_*,B_*,\eta),\ u(M\ |\ \eta )\Big) \Bigg]$.
%\begin{align}\label{eq:loss}
 %   \mathcal{C}\big(M\   |\ A_*, B_* \big)=\mathbb{E}_{\eta} \Bigg[ c\Big(x(M\ |\ A_*,B_*,\eta),\ u(M\ |\ \eta )\Big) \Bigg].
%\end{align}
$\mathcal{C}$ is a convex function of $M$, because $x$ and $u$ are affine in $M$ and $c$ is convex. We define the policy set
\begin{align}\label{eq:policy-set}
    \mM=\left\{\left(M^{[0]},\dots,M^{[H-1]}\right) \ \Big|\ \left\|M^{[i]}\right\|\leq \kappa^3\beta (1-\gamma)^i \right\}.
\end{align}
The following theorem captures that $\mM$ can approximately express all policies in $\mathcal{K}$.% \op{put definition of $\M$ somewhere else}

\begin{theorem}[\cite{agarwal2019online}]\label{thm:cvx_relax}
For all $K\in \mathcal{K}$, there exists a disturbance-based policy $M\in \mathcal{M}$, such that $\Big|\mathcal{C}\left(M\   |\ A_*, B_* \right)-J(K)\Big|\leq 1/T$.
\end{theorem}
The theorem above is a slight modification of a result proved in \cite{agarwal2019online}, and we provide its proof in Appendix \ref{appdx:prf:thm:cvx-relax}.
The algorithms we present in the paper, aim to minimize the function $\mathcal{C}\left(M\   |\ A_*, B_* \right)$. The difficulty is that we don't know this function, since we don't know $A_*,B_*$.

\subsubsection{Barycentric spanners}
Barycentric spanners and approximate barycentric spanners were introduced in \cite{awerbuch2008online}. Here, we will use the affine version of approximate barycentric spanners, defined below.

\begin{definition}\label{def:barycentric}
 Let $K$ be a compact set in $\mathbb{R}^d$. A set $X = \{x_0,x_1, \dots , x_d\}\subseteq K$ is a $C$-approximate affine barycentric spanner for $K$ if every $x \in  K$ can be expressed as $x=x_0+\sum_{i=1}^d\lambda_i(x_i-x_0)$, where the coefficients $\lambda_i\in[-C,C]$.
\end{definition}
%Here, we use the affine versions of the above definitions, i.e., affine barycentric spanners and $C$-approximate affine barycentric spanners. The definitions are the same as above, except that the linear combinations are replaced with affine combinations and the set $X$ has $d+1$ elements, instead of $d$.
The above theorem follows from Proposition 2.5 in \cite{awerbuch2008online}, as we show in Appendix \ref{appdx:prf:thm:lin-opt-oracle}.% \op{fix thm}
\begin{theorem}\label{thm:lin-opt-oracle}
Suppose $K\subseteq \mathbb{R}^d$ is compact and not contained in any proper affine subspace.  Given an oracle for optimizing linear functions over $K$, for any $C > 1$ we can compute a $C$-approximate affine barycentric spanner for $K$ in polynomial time, using $O(d^2 \log_C(d))$ calls to the oracle.
\end{theorem}

%\begin{definition}
 %Let $K$ be a compact set in $\mathbb{R}^d$. A set $X = \{x_0,x_1, \dots , x_d\}\subseteq K$ is a $C$-approximate affine barycentric spanner for $K$ if every $x \in  K$ can be expressed as an affine combination of elements of $S$ using coefficients in $[−C,C]$.
%\end{definition}

%\paragraph{Surrogate regret:} 
%Let $$

%\begin{align}\label{eq:loss}
    %\mathcal{C}\left(M\   |\ A_*, B_* %\right)=\mathbb{E}_{\eta} \Bigg[ c\Big(x(M\ |\ A_*,B_*,\eta),\ u(M\ |\ \eta )\Big) \Bigg]
%\end{align}
%$\mathcal{C}$ is a convex function of $M$, because $x$ and $u$ are linear in $M$ and $c$ is convex.

%\begin{theorem}[\cite{agarwal2019online}]\label{thm:cvx_relax}
%With high probability, $|\widetilde{R}_T-R_T|\lesssim 1$.\footnote{To be precise, the result from \cite{agarwal2019online} needs to be combined with the standard fact that with high probability $\|w_t\|\leq \widetilde{O}\left(\sqrt{d_x}\right)$, for all $t$, to get the theorem that we state.}
%\end{theorem}
%\begin{claim}\label{cl:inf_loss-stat_loss}
%For all $M\in \mM$, $|\mL(M|A_*,B_*)-J(M)|\lesssim 1/T$.
%\end{claim}
%\begin{proof}
%todo
%\end{proof}
%If a perturbation-based policy $M$ is used for all steps, we will refer at the state and control at time $t$ as $x_t(M)$ and $u_t(M)$. 
%In \cite{agarwal2019online}, the authors prove that noise-based policies can approximately express all policies in $\mathcal{K}$. We give some definitions and then we state their theorem. First, let
%\begin{align}
 %   \mM=\left\{\left(M^{[0]},\dots,M^{[H-1]}\right) \ \Big|\ \|M^{[i]}\|\leq \kappa^3\theta (1-\gamma)^i \right\}
%\end{align}
%\paragraph{Surrogate Regret:}
%The surrogate regret is defined with respect to the set of noise-based policies $\mathcal{M}$:
%\begin{align}
 %   \widetilde{R}_T=\sum_{t=1}^T c(x_t,u_t) - T\min_{M\in \mathcal{\mM}}J(M)
%\end{align}
%where $J(M)=\lim_{T\to \infty} \frac{1}{T}\mathbb{E}_M\left[\sum_{t=1}^Tc\left(x_t,u_t\right)\right]$, and $\mathbb{E}_M$ is the expectation under policy $M$.

%\begin{theorem}[\cite{agarwal2019online}]\label{thm:cvx_relax}
%With high probability, $|\widetilde{R}_T-R_T|\lesssim 1$.\footnote{To be precise, the result from \cite{agarwal2019online} needs to be combined with the standard fact that with high probability $\|w_t\|\leq \widetilde{O}\left(\sqrt{d_x}\right)$, for all $t$, to get the theorem that we state.}
%\end{theorem}
%From now on, the $H$ that we will be as in the above Theorem. Under the execution of a stationary policy $M$, the state may be expressed as a linear transformation $\Psi$ (defined below) of the perturbations, where transformation $\Psi$ is is linear in the matrices of $M$.
%By unrolling $x_{t+1}(M)$ we get
%\begin{align}
    %x_{t+1}(M)=A_*^{H+1}x_{t-H}+\sum_{i=0}^{2H}\Psi%_i(M)w_{t-i}
%\end{align}

%\begin{align}\label{eq:transfer}
    %\Psi_i(M)=A_*^i\ind_{i\leq H}+\sum_{j=0}^HA_*^j %B_* M^{[i-j-1]}\ind_{i-j\in[1,H]}
%\end{align}
%\includegraphics[width=\linewidth]{7.png}

%Given a policy $M$ and a sequence $w_{1:H}=(w_0,\dots,w_{2H})$ we define a surrogate state and surrogate control as follows.

%\includegraphics[width=\linewidth]{9.png}
%\begin{align}\label{eq:sur_state}
   % x(M|A_*,B_*,w_{0:2H})=\sum_{i=0}^{2H}\Psi_i(M)w_i
%\end{align}
%\begin{align}\label{eq:sur_control}
 %   u(M|w_{0:H-1})=\sum_{i=0}^{H-1}M^{[i]}w_i
%\end{align}
%Observe that there is no time dependence in the above two equations. The reason is that $w_t$ are iid, so we will not need a time-dependent definition.
%\par 
%{\color{red} use the stationary term in the other contexts too}\\
%Moreover, we define the following stationary loss on a policy $M$:


%\begin{align}\label{eq:loss}
 %   \mL\left(M   | A_*, B_* \right)=\mathbb{E}_{w_{0:2H}}\ell\left(x(M|A_*,B_*,w_{0:2H}),u(M|w_{0:H-1}\right)
%\end{align}
%where $w_0,\dots,w_{2H}\sim N(0,I)$ and independent. This loss is \emph{convex}, since $y$ and $v$ are linear in $M$, $\ell$ is convex, so we get an average of convex losses, which is convex.

%\begin{claim}\label{cl:inf_loss-stat_loss}
%For all $M\in \mM$, $|\mL(M|A_*,B_*)-J(M)|\lesssim 1/T$.
%\end{claim}
%\begin{proof}
%todo
%\end{proof}

==> discussion.tex <==
\section{Discussion and open questions}
sources of dimension dependence and improvements: improve $d^{3/2}$ if you have info about $\ell$, do the right exploration, compete with better than linear policies. Adversarial case. Partial observation?

==> extensions.tex <==
\section{Extensions}\label{sec:extensions}
Initial stable policy, subgaussian noise+we don't need noise simulator, can use noise approximations, quadratic costs=lipscitz in proper region, $\ell(0,0)\leq 1$ unecessary (maybe you don't have to do this one)


==> gradient-method.tex <==




\section{Gradient Perturbation Controller}

\paragraph{LDS setting.}
Consider a sequence of adversarial loss functions $c_{1:T}$ with  full feedback. We have the following dynamics in the background. 
$$ x_{t+1} = A x_t + B u_t + w_t ,$$ 
where $A,w_t$ are unknown, but $B$ is known and $x_t$ is observed at the $t$'th iteration. A stabilizing controller $K$ is given. 
Further it is assumed that $w_t \sim N(0,1)$ are i.i.d. Gaussian. 

\paragraph{The convex relaxation from non-stochastic control.}
The dynamics equation can be re-written as
$$ x_{t+1} = \sum_{i=0}^t A^i (B u_{t-i} + w_{t-i}) $$ 
Now using the convex relaxation $u_t = K x_t + M^t_{1:h} w_{t:t-h} $, where we denote $w_{t:t-h} = (w_t,...,w_{t-h})$ and similarly for $M$, we have 
\begin{align*}
x_{t+1} & = \sum_{i=0}^t (A+BK)^i (B  M^{t-i}_{1:h} w_{t-i:t-i-h} + w_{t-i} ) \\
&\approx_\eps \sum_{i=t-H}^t (A+BK)^i (B  M^{t-i}_{1:h} w_{t-i:t-i-h} + w_{t-i} ) \\ 
& =  \sum_{i=t-H}^t M^{t-i}_{1:h} C^{t-i}_{1:h}  + C^{t-i}_0  
\end{align*}
where $H=H(\eps)$ is the effective memory length determined by the desired accuracy and the condition number of the system. If $\|A\| \leq 1-\delta$, then $H = O(\frac{1}{\delta} \log \frac{1}{\eps})$. In addition, the coefficients $C^t_{1:h} $ are as follows, where $N_i = (A+BK)^i B$. 
$$ C^{t-i}_0 =  N_i w_{t-i} \ , \  C^{t-i}_j = N_i B w_{t-i-j} . $$ 



\paragraph{Loss reformulation w. memory.}

Thus, we can rewrite the costs as a function of $M$ as follows
$$ c_t(x_t(M),u_t(M)) = c_t( M^{t:t-H}_{1:h} C^{t:t-H}_{1:h}  ) = f_t( M^{t:t-H}_{1:h} ) . $$ 

As in the paper of loss functions with memory, we abuse notation and write 
$$f_t(M_{1:h}) = f_t(M) = f_t(M^{t:t-H}_{1:h} C^{t:t-H}_{1:h}  | M^{t-i} = M)  . $$

\subsection{The algorithm} 

\begin{algorithm}
\begin{algorithmic}[1]
\STATE Input: horizon $T$, initial point $x_1$, $B$, stabilizing  $K$ 
\FOR{$t = T_1+ 1, \ldots, T$}
\STATE Observe $x_t$, play $u_t = K x_t + M^t \hat{w}_{t:t-h} $
\STATE Create {\bf unbiased}  estimate of $A,w_t,N_i$ by 
$$ \hat{A}_t = \argmin_{A} \left\{ \sum_{\tau=1}^{t-H} \|x_\tau - A x_{\tau -1} - B u_{\tau  - 1}\|^2 \right\}   \ , \ \hat{w}_t = x_t - \hat{A}_t x_{t-1} - {B} u_{t-1} $$
$$ \hat{N}_i^t = \prod_{j=1}^i \left( \argmin_{A} \left\{ \|x_{t-j} - A x_{t-j -1} - B u_{t-j  - 1}\|^2 \right\} + BK \right)   $$

\STATE Update estimates $\hat{C}^t$ using $\hat{N}_i^t,\hat{w}_\tau$,
update $x_t$ via OGD and gradient estimate $\hat{\nabla_t} = f_t'(M^t \hat{C}^t ) \hat{C}^t $
$$ M^{t+1} = \prod_\K \left[ M^t - \eta \hat{\nabla_t} \right] $$
\ENDFOR
\end{algorithmic}
\end{algorithm}


\subsection{Regret bound}

\begin{theorem}
$$ \sum_t f_t(M^t) -f_t(M^*)  = O(\sqrt{T} ) $$ 
\end{theorem}
\begin{proof}


Henceforth we let $\hat{f}_t(M) = f_t(M^{t:t-H}_{1:h} \hat{C}^{t:t-H}_{1:h}  | M^{t-i} = M)$.  
\begin{lemma}[Simulation Lemma from RL]
$$ f_t(M_t) = \hat{f}_t(M_t)$$
\end{lemma}
This lemma says that the cost we pay according to the fictitious world view that we have created is equal to the real cost according to the real cost function. It is true since the states we observe are true regardless of the interpretation we give to how they were created (estimations of perturbations and the system). 



Due to the OGD analysis, we have of course that even accounting for memory,
$$ \sum_t \hat{f}_t(M^t) - \sum_t \hat{f}_t(M^*) = O(\sqrt{T}) .$$

The following lemma follows from Cohen et al and Orestis writeup:
\begin{lemma}
$$ \sum_t \| \hat{w}_t - w_t \| = O(\sqrt{T} ) $$ 
\end{lemma}



\paragraph{Notation.}
We henceforth denote $\hat{C}$ - estimates of $C$ with estimates $\hat{A},\hat{B},\hat{w}$. Let $\tilde{C}$ be estimates of $C$ with real ${w}$ but estimates $\hat{A},\hat{B}$. Similarly, we let $\hat{f}$ be $f(M\hat{C})$, and $\tilde{f} = f(M \tilde{C})$.


\begin{eqnarray*}
& \sum_t{f}_t(M^t) - \sum_t  {f}_t(M^*) \\
& = \sum_t ( \hat{f}_t(M^t) -  \hat{f}_t(M^*) )
 + \sum_t ( \hat{f}_t(M^t) - {f}_t(M^t)) 
 + \sum_t ( {f}_t(x^*) -  \hat{f}_t(M^*)) \\
& = O(\sqrt{T})  + 0   + \sum_t ( {f}_t(M^* C^t) -  {f}_t(M^* \hat{C}^t )) ) & \mbox{simulation lemma} \end{eqnarray*}

We now bound the latter term. Recall $N_i = (A+BK)^i B$, and $\hat{N}_i = (\hat{A}+\hat{B}K)^i \hat{B}$.
 By definition, 
$$ C^{t-i}_j = N_i w_{t-i-j} \ , \ \hat{C}^{t-i}_j = \hat{N}_i \hat{w}_{t-i-j} \ , \ \tilde{C}^{t-i}_j = \hat{N}_i {w}_{t-i-j} . $$
Continuing the computation from before, 
\begin{eqnarray*}
& \sum_t{f}_t(M^t) - \sum_t  {f}_t(M^*) -  O(\sqrt{T}) = \sum_t  {f}_t(M^* C^t) -  {f}_t(M^* \hat{C}^t ) \\
& = \sum_t  {f}_t(M^* C^t) - {f_t}(M^*\tilde{C}^t) + {f}_t(M^* \tilde{C}^t) -  {f}_t(M^* \hat{C}^t ) \\
& \leq \sum_t  {f}_t'(M^* C^t)( M^* C^t - M^*\tilde{C}^t) + {f}'_t(M^* \tilde{C}^t) ( M^* \tilde{C}^t - M^* \hat{C}^t ) \\
& \leq \sum_t  {f}_t'(M^* C^t)( M^* C^t - M^*\tilde{C}^t) + L \|  M^* \tilde{C}^t - M^* \hat{C}^t \| \\
& \leq \sum_t  {f}_t'(M^* C^t)( M^* C^t - M^*\tilde{C}^t) + L \|  w_t - \hat{w}_t \| \\
& \leq \sum_t  {f}_t'(M^* C^t)( M^* C^t - M^*\tilde{C}^t) + O(\sqrt{T}) \\
& \leq \sum_t  {f}_t'(M^* C^t)( M^* N^{t:t-h} w^{t:t-h} - M^* \hat{N}^{t:t-h} w^{t:t-h}) + O(\sqrt{T}) 
\end{eqnarray*}
Notice that $C^t$ is independence on $N^t$, and we can therefore have
$$ \E[  \sum_t  {f}_t'(M^* C^t)( M^* N^{t:t-h} w^{t:t-h} - M^* \hat{N}^{t:t-h} w^{t:t-h}) ] = 0 , $$ 
Since $\E[\hat{N} ] = N $, and the estimates of $N$ are independent of $w_t$ as well as on $M^*$. 


\end{proof}



==> intuition.tex <==
The algorithm runs in epochs and follows the phased-elimination paradigm \cite{lattimore_szepesvari_2020}. During epoch $r$, it focuses on a convex set of controls $\mathcal{U}_r$, which can be thought as an approximate sublevel set of $\mC(u\ |\ B_*)$, and which by the end of the epoch will be substituted by $\mathcal{U}_{r+1}\subseteq \mathcal{U}_r$, shrinking towards the optimal policy. Roughly, $\mathcal{U}_r$ is a sublevel set of $\mC(u\ |\ \widehat{B})$, where $\widehat{B}$ is an estimate of $B_*$, constructed using observations before the epoch $r$. To eliminate suboptimal policies from $\mathcal{U}_r$ and get $\mU_{r+1}$, it suffices to refine our estimate $\whB$ only in the directions relevant to the controls of $\mU_r$. To get these estimates, in the beginning of epoch $r$, the algorithm constructs a barycentric spanner of $\mathcal{U}_r$. As we explain in subsection \ref{}, this can be done in polynomial time, because we know the cost function $c$ and $\mU_r$ is convex. The elements of the spanner are the exploratory controls that we execute during the epoch and lead to generation of observations that give the information needed to refine $\whB$. 

==> old-intro.tex <==
\section{Introduction}
Adaptive control is the data-driven regulation of an unknown linear dynamical system \cite{bertsekas1995dynamic}. This paper studies adaptive control under general convex costs. 
In a linear dynamical system, the system state $x_t\in \mathbb{R}^{d_x}$ evolves as 
\begin{align}
    x_{t+1}=A_*x_t+B_*u_t+w_t,\ \ \ \text{where } x_1=0,
\end{align}
 $u_t\in \mathbb{R}^{d_u}$ is the learner's control input, $w_t\in \mathbb{R}^{d_x}$ is a noise process drawn as $w_t\simiid N(0,I)$\footnote{Our results hold for any subgaussian distribution.}, and $A_*,B_*$ are unknown system matrices with the implied dimensions. The learner receives implicit information about $A_*,B_*$, by applying $u_t$ at timestep $t$ and then observing $x_{t+1}$. At time $t$, she suffers cost $c(x_t,u_t)$, where $c$ is a convex function. We consider two different models. 

\begin{enumerate}
    \item Full cost information: the learner knows the cost function $c$ in advance.
    \item Bandit feedback: the learner does not know the cost function in advance, but observes at time $t$ the current cost $c(x_t,u_t)$.
\end{enumerate}

 The policy class we consider are \emph{stable linear policies}. Each linear policy is parameterized by some matrix $K$, and the control it generates at time $t$ is $u_t=Kx_t$. It is called stable if the spectral radius $\rho\left(A_*+B_*K\right)<1$. The goal of the algorithm is to iteratively choose controls $u_t$ for $T$ time steps, and minimize regret against the class of all stable linear policies. 
 \par The challenge is that initially the system matrices $A_*,B_*$ are unknown, making adaptive control a Reinforcement Learning (RL) problem with continuous state and control spaces. In RL theory, the tabular setting (discrete states and actions) is relatively well-understood \cite{}. For continuous spaces, provable guarantees and polynomial-time algorithms have been more elusive, and progress is spread across various models \cite{}. To the best of our knowledge, none of these models encompasses adaptive control  {\color{red} check}. The difficulty is balancing exploration and exploitation: should the algorithm play controls with uncertain outcomes to explore the system (e.g. random controls) or exploit, i.e. apply the control that looks best based on current data?
 
\par
Regret guarantees for adaptive control have been a subject of intense recent interest, both for the special case where the cost function is convex quadratic \cite{}, and for general convex costs \cite{}.
The case of quadratic costs is the classical linear quadratic regulator and is frequently used, even when it is not entirely justified, because it leads to a nice analytical solution when the system is known \cite{bertsekas1995dynamic}. However, this modeling choice is fairly restrictive, as opposed to general convex costs that can model constraints on state or restrictions that make the current set of available controls depend on
the current state. In practice, imposing constraints is crucial for control in order to ensure safe operating conditions.
\par
The existing algorithms and their regret bounds for adaptive control under general convex costs are unsatisfying. The best known regret bound is $T^{2/3}$ \cite{}. Furthermore, even though the whole bandit and RL theory literature is about sophisticated and sample-efficient exploration, the only algorithms we know for this problem are variants of the simplest exploration strategy: $\epsilon$-greedy, known in control literature as certainty equivalence. In contrast to the general case,  $\epsilon$-greedy achieves $\sqrt{T}$-regret for \emph{strongly-convex} costs \cite{}, and this is optimal \cite{}. These results heavily rely on strong convexity and to tackle the general case we need to go beyond $\epsilon$-greedy. We aim to answer the following question:
\\
\\
\emph{Can we design sample-efficient exploration algorithms for adaptive control under general convex costs?}
\\

\par
We answer this question in the affirmative by designing the first polynomial-time algorithms that achieve $\sqrt{T}$-regret for the two settings: full cost information and bandit feedback. Furthermore, we show that for the simpler case where matrix $B_*$ is known in advance, a simple online gradient descent-type algorithm achieves $\sqrt{T}$-regret. The fact that knowing $B_*$ greatly simplifies the problem was first noted in \cite{}.
\subsection{Our Results}
 In all theorems we write $p$ to express the polynomial dependence on natural system parameters.

\begin{theorem}[informal]\label{thm_inf:full-info}
For full cost information, with high probability, Algorithm \ref{LJ-exploration} achieves regret \footnote{ $\widetilde{O}(1)$ hides logarithmic factors.}
\begin{align}
    R_T\leq \widetilde{O}(1)\cdot p\cdot (d_xd_u)^{3/2}(d_x+d_u)\cdot \sqrt{T}.
\end{align}
\end{theorem}
\\

\begin{theorem}[informal]\label{thm_inf:bandit}
For bandit feedback, with high probability, Algorithm \ref{alg:bandit-feedback} achieves regret 
\begin{align}
    R_T\leq \widetilde{O}(1)\cdot p\cdot poly(d_x,d_u)\cdot \sqrt{T}.
\end{align}
\end{theorem}
\\

\\
\textbf{Comment:} In Theorem \ref{thm_inf:full-info} the polynomial dependence in the dimensions $d_x,d_u$ is rather large. This typically happens in bandit convex optimization (BCO) \cite{}. Our setting is more challenging than BCO, since the environment has a state.
\begin{theorem}[informal]\label{thm_inf:gradient}
When $B_*$ is known in advance, with high probability, Algorithm \ref{alg:gradient} achieves regret 
\begin{align}
    R_T\leq \widetilde{O}(1)\cdot p\cdot  poly(d_x,d_u)\cdot \sqrt{T}.
\end{align}
 {\color{red}add polynomial dependence in dimension}
\end{theorem}

Our main contribution is Algorithm \ref{LJ-exploration}, where we make a novel use of convex geometry to balance exploration and exploitation. To prove our results we introduce several new ideas that we summarize below.

\subsection{Our Approach and Contributions}

 For simplicity, we assume that the system is stable, i.e. the spectral radius $\rho(A_*)<1$. In section \ref{sec:extensions} we show how to relax this assumption, in accordance with previous works. Our algorithms, instead of working with stable linear policies, they use noise-based policies \cite{ } of the form 
\begin{align}\label{eq:noise-based-policy}
  u_t=\sum_{i=1}^H M^{[i-1]}w_{t-i}, 
\end{align}
where $H$ is set appropriately. Instead of one matrix $K$, the policy is parameterized with a tuple of $H$ matrices: $M=\left(M^{[0]},\dots, M^{[H-1]}\right)$. Notice that the policy acts on the noises, instead of acting on the state. In \cite{}, the authors show that noise-based policies can approximate all stable linear policies. This parameterization is useful because at any time $t$, \emph{the cost as a function of the policy $M$ is convex}. This is in contrast with linear policies, where this cost is a nonconvex function\footnote{This nonconvexity is formally shown in \cite{}.}. From now on, when we only write "policy" we will mean noise-based policy. We move on to the novel components of our work.
\paragraph{John's exploration:} Algorithm \ref{LJ-exploration} runs in epochs and follows the phased-elimination paradigm \ref{}. During epoch $r$ it focuses on a \emph{convex} policy set $\mathcal{M}_r$, which by the end of the epoch will be substituted by the convex set $\mathcal{M}_{r+1}\subseteq \mathcal{M}_r$. Let's assume for the moment that the algorithm has access to the noises, in order to execute the policies as in \ref{eq:noise-based-policy}. We will drop this assumption momentarily. In the beginning of epoch $r$ it constructs a weak John ellipsoid of $\mathcal{M}_r$ (see Definition \ref{}). Then, it chooses the center and the axes of the ellipsoid to be the \emph{exploratory policies}, i.e. the policies that it will execute during this epoch to collect useful data. Using these data, it estimates the system matrices $A_*,B_*$ and creates $\mathcal{M}_{r+1}\subseteq \mathcal{M}_r$. For the implementation, to efficiently compute the ellipsoids we use a classical algorithm of Lovasz \cite{}, which we show how to further modify to improve the regret. To the best of our knowledge, our adaptive exploration strategy is different from prior uses of weak John ellipsoid and we make a comparison in section \ref{}.
\paragraph{Noise approximation:} Now, we drop the assumption that we know the noises $w_t$, by computing approximations $\widehat{w}_t$ and using these instead. Previous works \cite{} compute these by first approximating the system matrices in spectral norm. To do this, they play random controls (e.g. $u_t\sim N(0,I)$) for several steps and thus compromise in terms of cost. A key contribution of this work is showing that \emph{noise approximation can be done without accurately learning the system matrices}. Specifically, we show that for any choice of controls $u_t$, we can get $\widehat{w}_t$ such that $\sum_{t=1}^T \|\widehat{w}_t-w_t\|^2 \leq  \widetilde{O}(1)\cdot (d_x+d_u)^3$. This inequality alleviates all issues arising from not knowing the true noises $w_t$.
\paragraph{Coupling:} At the end of epoch $r$, we create estimates $\whA,\whB$ of $A_*,B_*$, which we use to create the next policy set $\mathcal{M}_{r+1}$. These estimates are not necessarily accurate in every direction. To argue that $\mathcal{M}_{r+1}$ contains good policies we employ a probabilistic coupling argument between the true system and the estimated one. This could be a useful technique for future works.

\paragraph{Robustness of stochastic BCO:} For the case of bandit feedback, we apply bandit convex optimization (BCO) in policy space. To do this, we define a generalization of the stochastic BCO framework, where the noise is stochastic plus a small adversarial component. Although we are aware of such models for multiarmed and linear bandits \cite{}, to the best of our knowledge this is the first for convex bandits. We prove that by appropriately changing only one hyperparameter in the stochastic BCO algorithm from \cite{}, we can get $\sqrt{T}$-regret for this model. The need for robustness to adversarial perturbations arises from the approximation error on the noises $\|\widehat{w}_t-w_t\|$. However, because of the noise-approximation analysis, these perturbations are small and the aforementioned algorithm can be used for control with bandit feedback.

%\subsection{Our Contributions}
%To achieve these results we introduce new ideas and we make several technical contributions.
%\begin{itemize}
 %   \item For full cost information, we use tools from convex geometry to balance exploration and exploitation. In particular, we adaptively construct a sequence of "weak John ellipsoids" \cite{lovasz1990geometric} in an over-parameterized policy space. These ellipsoids determine which policy will be executed at each step. To the best of our knowledge, this adaptive construction is novel and we compare it with prior uses of John ellipsoid in section \ref{}. Moreover, we show that changing the classical algorithm of Lovasz \cite{} for computing these ellipsoids improves the sample efficiency.
    
  %  \item We prove a key lemma on the online recovery of the unobserved noise vectors $w_t$. We show that \emph{accurate recovery of the noise vectors does not require exploration of the system matrices}. This lemma might be of independent interest. We note that prior works \cite{} first recover the system matrices and then the noises.
    
   % \item For full cost information, the algorithm does not estimate uniformly all directions of $A_*,B_*$. To argue that the constructed estimates lead to good policies, we employ a probabilistic coupling argument between the true system and the estimated one. This could be a useful technique for future works.
    
    %\item For bandit feedback
%\end{itemize}                     



\\
\\
\\





\subsection{Prior Work}
put mpc for constraints, rockafellar, john ellipsoid + appl in bandits
explain that benefit of this relaxation is that you don't worry about state explosion: Cohen et al. really need to take into account of this.  

\subsection{Organization}
\subsection{Preliminaries}
For all $t$, let $z_t=\begin{pmatrix} x_t \\ u_t\end{pmatrix}$.
To put: Matrix inner product,$\lesssim$,
$\tilde{O} $ meaning, $\|\cdot\|$ for vectors is $\ell_2$ norm, for matrices operator. Forbenius norm. Also align paper with these. Det =$||$. Explain what whp will mean and apply it. Explain $w_{i:j}$ notation. Clarify $\tilde{O}$, $H=\tilde{\Theta}(...)$, like for example the choice of H.
Argue why we are different in john ellipsoid linear bandits, convex bandits.


==> prio-work-elad.tex <==
\paragraph{Geometric exploration and BCO.} The main novelty in our work relates to exploration in improper convex relaxations for learning. This relates to a large literature on bandit convex optimization, the reader is referred to the texts \cite{bubeck2012regret,lattimore_szepesvari_2020}. Volumetric spanners and John ellipsoids were used for exploration in the context of {\it proper} bandit optimization in \cite{hazan2016volumetric,bubeck2012towards} and an online stochastic ellipsoid method use developed in \cite{agarwal2011stochastic}.



\paragraph{Online Control of LQR} When the cost $c$ is convex quadratic, we obtain the online LQR setting. For a survey of the field of online and adaptive control see \cite{stengel1994optimal}. 
Low regret in the online LQR setting with known systems was studied in \cite{abbasi2011regret,dean2018regret,mania2019certainty,cohen2019learning} where a fully-observed linear dynamic system is drive by i.i.d. Gaussian noise, and the learner incurs constant quadratic state and input cost. Recent algorithms \cite{mania2019certainty,cohen2019learning} attain $\sqrt{T}$ regret for this setting, with polynomial runtime and polynomial regret dependence on relevant problem parameters. 

\cite{cohen2018online} establish $\sqrt{T}$ in  a variant of online LQR where the system is known to the learner, noise is stochastic, but an adversary selects quadratic loss functions at each time. 
Provable control in the Gaussian noise setting via the policy gradient method was  studied in \cite{fazel2018global}. Other relevant work from the machine learning literature includes the technique of spectral filtering for learning and open-loop control of partially observable systems \cite{hazan2017learning, arora2018towards, hazan2018spectral}, as well as prior work on tracking adversarial targets \cite{abbasi2014tracking}.



\paragraph{Non-stochastic control.}
The convex relaxation we consider in this paper was established in 
\cite{agarwal2019online}, who obtain $\sqrt{T}$-regret in the more general and challenging setting where the Lipschitz loss function \emph{and the perturbations } are adversarially chosen. The key insight behind this result is combining an improper controller parametrization know as disturbance-based control with recent advances in online convex optimization with memory due to \cite{anava2015online}. Follow up work by \cite{agarwal2019logarithmic} achieves logarithmic pseudo-regret for strongly convex, adversarially selected losses and well-conditioned stochastic noise. Under the considerably stronger condition of controllability, the recent work by \cite{Hazan2019TheNC} attains $T^{2/3}$ regret for adversarial noise/losses when the system is \emph{unknown}. Analogous problems have also been studied in the tabular MDP setting \cite{even2009online,zimin2013online,dekel2013better}.


\paragraph{Online learning and online convex optimization.}
We make extensive use of techniques from the field of online learning and regret minimization in games \cite{cesa2006prediction, shalev2012online, OCObook}. Of particular interest are techniques for coping with policy regret and online convex optimization for loss functions with memory \cite{anava2015online}. 

\paragraph{Linear System Identification:} To address unknown systems, we make use of tools from the decades-old field linear system identification~\cite{ljung1999system}. To handle partial observation and ensure robustness to biased and non-stochastic noise, we take up the approach in \cite{simchowitz2019learning}; other recent approaches include \cite{oymak2019non,sarkar2019finite,tsiamis2019finite,simchowitz2018learning}. 

==> trash.tex <==
\subsubsection{Regret analysis}\label{subs:acutal-regret}
In this subsection, we sketch a proof of Theorem \ref{thm:LJ-exploration}, using Lemma \ref{lem:loss_approx}.
\paragraph{Stationary regret:}
As we commented earlier, Algorithm \ref{LJ-exploration} tries to minimize $\mC(M|A_*,B_*)$. We define the \emph{stationary regret}, defined as
\begin{align}
    R_T^{st}=\sum_{t=1}^T\mC\left(M_t\ | \ A_*,B_*\right)-T\cdot\mC\left(M_*\ 
     |\ 
      A_*,B_*\right ),
\end{align}
where $M_t$ is the policy executed at time $t$ and $M_*\in \argmin_{M\in \mM}\mC(M\ |\ A_*,B_*)$. We will bound $R_T^{st}$, using Lemma \ref{lem:loss_approx}. After we sketch a proof of this bound, we will show that  $R_T-R_T^{st}$ is small.
\begin{lemma}\label{lem:stat-regret-bound}
With high probability, $R_T^{st}\leq \widetilde{O}\left(\gamma^{-3}\right)\cdot(d_xd_u)^{3/2}(d_x+d_u)
\sqrt{T}$.
\end{lemma}
%we can prove that the elimination step of Algorithm \ref{LJ-exploration} (equation \ref{eq:elimination}) rules out $O(2^{-r})$-suboptimal policies and keeps the optimal ones, which concludes the proof of Lemma \ref{lem:regr_each_step}. The proof of Lemma \ref{lem:loss_approx} is the main component of our analysis.

To bound $R_T^{st}$, we first observe that if $t$ is in epoch $r$, then $M_t\in \mM_r$. We show that the policy set $\mM_r$ "improves" exponentially in each epoch. Concretely, we prove the following lemma.

\begin{lemma}\label{lem:regr_each_step}
Let $R^{st}(M)=\mC(M\ |\ A_*,B_*)-\mC(M_*\ |\ A_*,B_*)$. With high probability, for all epochs $r>1$ and $M\in \mM_{r}$, we have $R^{st}(M)\lesssim 2^{-r}$.
\end{lemma}
Given Lemma \ref{lem:regr_each_step}, we have a guaranteed improvement of the executed policies, and after some calculations (given in Appendix \cite{}), we can prove Lemma \ref{lem:stat-regret-bound}. Lemma \ref{lem:regr_each_step} is an implication of Lemma \ref{lem:loss_approx}: since cost is estimated with error $2^{-r}$, the elimination step of Algorithm \ref{LJ-exploration} (equation \ref{eq:elimination}) rules out all $\Omega(2^{-r})$-suboptimal policies ($R^{st}(M)\geq \Omega(2^{-r})$), while keeping the optimal policy $M_*$, which concludes the proof of Lemma \ref{lem:regr_each_step}.

\subsubsection*{Actual regret}
We bound $R_T-R^{st}_T$ to control the actual regret $R_T$. Let $K_*\in \argmin_{K\in \mathcal{K}} J(K)$.
To simplify notation, we use $\mC(M_t)$ to denote $\mC(M_t\ |\ A_*,B_*)$.
\begin{align}
R_T-R^{st}_T&= \sum_{t=1}^T \Big(c(x_t,u_t)- \mC(M_t) \Big) +T\Big(\mC(M_*) -J(K_*)\Big) \notag \\
  &  \lesssim \sum_{t=1}^T \Big(c(x_t,u_t)- \mC(M_t\ ) \Big)+1,
\end{align}
where we used Theorem \ref{thm:cvx_relax}. To bound the above sum, we introduce the auxiliary state/control sequence defined as
\begin{align}\label{eq:sur_state}
    \ox_t =\sum_{i=1}^{H}A_*w_{t-i}+\sum_{i=1}^{H}A_*B_*\ou_{t-i}\ \ \ \ \text{and}\ \ \ \ou_t=\sum_{i=1}^HM_t^{[i-1]}w_{t-i}.
\end{align}

  Compare the above with $x_t=A_*^{H+1}x_{t-H+1}+\sum_{i=1}^{H}A_*w_{t-i}+\sum_{i=1}^{H}A_*B_* u_{t-i}$ and $u_t=\sum_{i=1}^HM_t^{[i-1]}\widehat{w}_{t-i}$. The differences are that in $(\ox_t\ \overline{u})$ 1) the time horizon is truncated. i.e., the term $A_*^{H+1}x_{t-H+1}$ is missing and 2) the controls use the true perturbations instead of estimates. We have
\begin{align}\label{eq:decomp-martingale}
\sum_{t=1}^T \Big(c(x_t,u_t)- \mC(M_t) \Big)&= \sum_{t=1}^T \Big(c(\ox_t,\ou_t)- \mC(M_t)\Big) +\sum_{t=1}^T \Big(c(x_t,u_t)- c(\ox_t,\ou_t) \Big).
\end{align}
We bound the two sums with the following lemmas.

\begin{lemma}\label{lem:surrogate-state-bound}
With high probability, 
 \begin{align}
     \sum_{t=1}^T \Big(c(x_t,u_t)- c(\ox_t,\ou_t) \Big)\leq \widetilde{O}\left(\kappa^5\beta^2\gamma^{-2}\right)\cdot (d_x+d_u)^{3/2}\sqrt{T}.
 \end{align}
\end{lemma}
\begin{proof-sketch}
 We have $c(x_t,u_t)- c(\ox_t,\ou_t)\leq \|(x_t\ u_t) - (\ox_t\ \ou_t)\|$, since  $c$ is 1-Lipschitz. By subtracting the two state/control sequences and doing some calculations we get
 \begin{align}\label{eq:sur_state-bound}
      \left\|(x_t\ u_t) - (\ox_t\ \ou_t)\right\|\lesssim 1/T+ \widetilde{O}\left( \kappa^5\beta^2\gamma^{-1} \right)\cdot  \sum_{i=1}^{2H+1}\|\whw_{t-i}-w_{t-i}\| 
 \end{align}
These two terms correspond to the two differences that we mentioned above. The term $1/T$ appears because $\|A_*^{H+1}x_{t-H+1}\|$ can be shown to be $O(1/T)$, because of Assumption \ref{assump:stability}. Furthermore, Lemma \ref{lem:noise-approx} followed by Cauchy-Schwarz gives $\sum_{t=1}^T\|\whw_{t}-w_{t}\|\leq (d_x+d_u)^{3/2}\sqrt{T}$. Summing inequality \ref{eq:sur_state-bound} over all $t$ finishes the proof.
\end{proof-sketch}
\begin{lemma}\label{lem:martingale}
With high probability, 
 \begin{align}
     \sum_{t=1}^T \Big(c(\ox_t,\ou_t)- \mC(M_t)\Big)\leq \widetilde{O}\left(\kappa^5\beta^2\gamma^{-3}\right)\cdot \sqrt{T}
 \end{align}
\end{lemma}
\begin{proof-sketch}
Let $I$ be the set of timesteps $t$ such that $M_{t-H-1}=M_{t-H}=\dots =M_t$. For all $t\in I$, $(\ox_t\ \ou_t)$ has the same distribution as the surrogate state/control pair defined in \ref{eq:sur_state}. Thus, if $t\in I$, then $\mathbb{E}[c(\ox_t,\ou_t)]= \mC(M_t)$. We apply concentration bounds to show that $\sum_{t\in I }(c(\ox_t,\ou_t)- \mC(M_t))\leq \widetilde{O}\left(\kappa^5\beta^2\gamma^{-3}\right)\cdot \sqrt{T}$. The rest of the sum is bounded by using the fact that the size of the set $[T]\setminus I$ is small, i.e., logarithmic in $T$, which can be seen by inspecting Algorithm \ref{LJ-exploration}. 
\end{proof-sketch}
The above bounds, combined with Lemma \ref{lem:stat-regret-bound} give the desired bound on $R_T$ and conclude the proof of Theorem \ref{thm:LJ-exploration}.



\subsection{Proof overview}
As in Section \ref{sec:known-cost}, we separately bound the stationary regret $R_T^{st}$ and the difference $R_T-R_T^{st}$. Here, we sketch the bound for $R_T^{st}$ and we give complete proofs for both bounds in the Appendix. The function that plays here the role of $f$ in the SBCO setting is $\mC(M\ |\ A_*,B_*)$. When the SBCO algorithm queries a point/policy $M$, Algorithm \ref{alg:bandit-feedback} executes $M$ for $2H+1$ steps and then sends $c(x_t,u_t)$ to the SBCO algorithm. To see why this is a natural attempt to implement the noisy value oracle, suppose momentarily that $\whw_{s}=w_{s}$ for all $s$. Then, we have $u_t=\sum_{i=1}^HM^{[i-1]}w_{t-i}$ and $x_t=A_*^{H+1}x_{t-H-1}+\sum_{i=1}^{2H+1}\Psi_i(M\ |\ A_*,B_*)w_{t-i}$. Without the the term $A_*^{H+1}x_{t-H-1}$, the cost $c(x_t,u_t)$ would have been an unbiased and independent estimate of $\mC(M\ |\ A_*,B_*)$. As we pointed in previous sections, $A_*^{H+1}\approx 0$, so this form of bias is easy to handle. A more subtle bias comes from the errros $\|\whw_s-w_s\|$. We can show that with high probability, $\sum_{t=1}^T \|\widehat{w}_t-w_t\|^2\leq \widetilde{O}(1)\cdot (d_x+d_u)^3$, by applying the same proof with Lemma \ref{lem-main:noise-approx}. However, it is not a priori clear that the SBCO algorithm of \cite{agarwal2011stochastic} is robust to biases that are small only on average. In the full proof, we show that by appropriately setting the input variance parameter $\sigma^2$, the SBCO algorithm achieves $\sqrt{T}$- regret even in the presense of these biases, which immediately gives a bound on $R_T^{st}$.

\begin{remark}[for experts in online optimization] 
It might seem more natural to use online bandit convex optimization (OBCO) \cite{}, instead of SBCO, to deal with the non-stochastic noise. The problem with the $\sqrt{T}$-regret algorithm of \cite{} is that it switches points many times, which breaks the bound on $R_T-R_T^{st}$. This is in contrast with the SBCO algorithm of \cite{agarwal2011stochastic}, for which the number of switches is only logarithmic in $T$.
\end{remark}

